Generate & Rank: A Multi-task Framework for Math Word Problems

Math word problem (MWP) is a challenging and critical task in natural language processing. Many recent studies formalize MWP as a generation task and have adopted sequence-to-sequence models to transform problem descriptions to mathematical expressions. However, mathematical expressions are prone to minor mistakes while the generation objective does not explicitly handle such mistakes. To address this limitation, we devise a new ranking task for MWP and propose Generate & Rank, a multi-task framework based on a generative pre-trained language model. By joint training with generation and ranking, the model learns from its own mistakes and is able to distinguish between correct and incorrect expressions. Meanwhile, we perform tree-based disturbance specially designed for MWP and an online update to boost the ranker. We demonstrate the effectiveness of our proposed method on the benchmark and the results show that our method consistently outperforms baselines in all datasets. Particularly, in the classical Math23k, our method is 7% (78.4% $\rightarrow$ 85.4%) higher than the state-of-the-art.

==> abs_old.tex <==
\begin{abstract}
Math word problem solving is a challenge and critical task in natural language processing. Recently, researchers have adopted Seq2Seq models to translate problem descriptions to mathematical expressions and achieved promising results. However, the translation task is not sufficient to obtain an accurate model since a single token change can cause the entire expression to be wrong. To address the problem, we propose to train a pre-trained generative language model under a multi-task framework, where the model can learn to 
rewrite and rank expressions from its own mistakes. The experimental results show that our model outperforms other methods and achieves a new state-of-the-art result.
\end{abstract}

==> approach_old.tex <==
\section{Methodolgy}

Figure \ref{fig:model} shows our proposed framework. 
(introduce the overall model and motivation)

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.90\textwidth]{fig/model-up.pdf}
    \caption{Caption}
    \label{fig:model}
\end{figure*}
\subsection{Multi-task Training}
\noindent {\bf Task #1: Generating}
The first task of our model is to generate expressions given a math word problem. This is a standard sequence-to-sequence task and we apply BART fine-tuning on MWP data directly. Specifically, the input to the encoder is a sequence of problem text tokens $P = (x_1, x_2, \dots, x_n)$ and the objective is to minimize the negative log-likelihood of the solution expression $S = (s_1, s_2, \dots, s_m)$.
\begin{equation}\label{eq:gen_loss}
    J_{gen} = \sum_{(P,S) \in D} -\log \Pr(S|P)
\end{equation}
where the conditional probability can be decomposed as:
\begin{align}
    \Pr(S|P) &= \prod_{i=1}^m \Pr(s_i|P, S_{j<i}) \\
    \Pr(s_i|P, S_{j<i}) &= softmax(d_iW + b) \\
    d_i &= BART_{Dec}(\mathbf{e};s_0, \dots, s_{i-1}) \\
    \mathbf{e} &= BART_{Enc}(x_1, x_2, \dots, x_n)
\end{align}
Following BART pre-training and fine-tuning, we add two special tokens $s_0 =$\textit{[bos]} and $s_m = $\textit{[eos]} to indicate the start and end of decoding sequences.

\noindent {\bf Task #2: Rewriting} 
Solving math word problems requires much more precision than other sequence-to-sequence tasks like summarization and translation, and training with the generation loss (\ref{eq:gen_loss}) alone may not be sufficient. Thus we design the rewriting task to make the model aware of mistakes in expressions and learn to fix them. The rewriting task is also a sequence-to-sequence task as generation, but with different input. Given a math word problem and an expression to rewrite, we concatenate them into one sequence, and add a separate token in between. In detail, we construct the input sequence in the following format: [P] Answer: [$\bar{S}$], where [P] is the problem text sequence, [$\bar{S}$] is the expression to rewrite, and ``Answer:'' is the separate token we add. The output sequence is the ground-truth expression $S$ of the problem, and the training objective of rewriting is negative log-likelihood as well as the generation.

\begin{equation}
    J_{rew} = \sum_{(P,S)\in D} \sum_{(P,\bar{S})\in D^-} -\log \Pr(S|P, \bar{S})
\end{equation}

Here we reuse the negative samples $D^-$ generated in verification for rewriting expressions.

\noindent{\bf Task#3: Ranking}
The verification is formulated as a sequence pair classification task. Given a pair of sequences of a problem and expression, the verifier should decide whether the expression is a correct solution to the problem or not. To achieve this, we add a new classifier on top of the final hidden state of the last decoder token. Note that the last decoder token is always the special \textit{[eos]} token and the corresponding hidden state can attend to all problem text and expression token representations. Same as the generation process, we feed the problem text into the encoder and the expression into the decoder, but we only need the output of the last decoder token and feed it into the classifier for prediction.
\begin{align}
    d_{m+1} &= BART_{Dec}(\mathbf{e};s_0,\dots, s_m) \\
    \Pr(\cdot|P,S) &= softmax(tanh(d_{m+1}W_1 + b_1)W_2 + b_2) \label{eq:verify}
\end{align}

The training objective of the verifier is the cross-entropy between the classifier output and the correctness label.
\begin{equation}
    J_{ver} = -\sum_{(P,S) \in D^+} \log\Pr(1|P,S) - \sum_{(P,S)\in D^-} \log\Pr(0|P,S)
\end{equation}
where $D^+$ and $D^-$ are sets of positive and negative pairs, respectively.
However, we only have positive (P, S) pairs (i.e., all expressions in our dataset are correct). In order to create negative samples, we use the previous trained generator with bean search to generate $K$ expressions for each problem, and evaluate them mathematically to give a numerical result. If the result matches with the groundtruth, this expression is labeled as positive, otherwise negative.

\noindent{\bf Training Objective}
We first fine-tune the pre-trained BART on sequence-to-sequence generation task ($J_{gen}$ in Eq. \ref{eq:gen_loss}). After that, we use this fine-tuned BART to generate expressions with beam search for negative samples in the verification and rewriting tasks. Then we train the model on the joint loss of all three tasks together
\begin{equation}\label{eq:joint_loss}
    J = J_{gen} + J_{rew} + J_{ver}
\end{equation}
and regenerate negative samples after each epoch. We summarize the whole training procedure in Algorithm \ref{alg:train}.

\begin{algorithm}[tb]
\caption{Training Algorithm}
\label{alg:train}
\textbf{Input:} MWP Dataset $D = \{(P,S)\}$ \\
\textbf{Parameter:} Pre-trained BART encoder and decoder parameters $\theta_e$ and $\theta_d$, random initialized verification classifier $\theta_v$

\begin{algorithmic}[1] %[1] enables line numbers
\STATE Fine-tune BART encoder $\theta_e$ and decoder $\theta_d$ on D with generation loss Eq. (\ref{eq:gen_loss}).
\STATE \textrm{// Generate negative samples}
\STATE $D^+ \gets D$, $D^- \gets \{\}$
\FOR{$(P,S) \in D$}
    \STATE Generate K expressions $\{\bar{S}_i\}$ for problem $P$ with beam search 
    \FOR{$\bar{S} \in \{\bar{S}_i\}$}
        \IF{$\bar{S}$ equals $S$}
            \STATE $D^+ \gets D^+ \cup \{(P,\bar{S})\}$
        \ELSE
            \STATE $D^- \gets D^- \cup \{(P,\bar{S})\}$
        \ENDIF
    \ENDFOR
\ENDFOR
\FOR{$epoch=1$ to $M$}
    \STATE Train $\theta_e$, $\theta_d$, $\theta_e$ w.r.t. the joint loss Eq.(\ref{eq:joint_loss}) on $D^+$ and $D^-$ 
    \STATE Repeat line. 3 - line. 13 to regenerate training samples
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Inference}
Given a new problem text sequence $P$, we first pass it to the encoder to get the problem representation $e$. Then we use the decoder log probability scores to perform beam search and choose top-K expressions. Each generated expression is concatenated with the problem text at the beginning and passed to the model again for rewriting. We also perform bean search for rewriting but only choose the top-1 expression. Finally, all the generated and rewritten expressions are passed to the verifier and one with the highest prediction score are selected as the final result. Algorithm \ref{alg:infer} shows the inference procedure.
\begin{algorithm}[!h]
\caption{Inference}
\label{alg:infer}
\textbf{Input:} A math word problem $P$

\begin{algorithmic}[1] %[1] enables line numbers
\STATE $\mathbf{e} \gets BART_{Enc}(P)$
\STATE $\{S_1, \dots, S_K \} \gets$ top-K beam search results starting from $BART_{Dec}(\mathbf{e};[bos])$
\STATE $\mathcal{S} \gets \{S_1, \dots, S_K \}$
\FOR{$i=1$ to $K$}
    \STATE $\hat{P} \gets$ concat(P, ``Answer:'', $S_i$)
    \STATE $\mathbf{\hat{e}} \gets BART_{Enc}(\hat{P})$
    \STATE $\hat{S} \gets$ top-1 beam search result starting from $BART_{Dec}(\mathbf{\hat{e}};[bos])$
    \STATE $\mathcal{S} \gets \mathcal{S} \cup \{\hat{S}\}$
\ENDFOR
\FOR{$s \in \mathcal{S}$}
    \STATE $d \gets BART_{Dec}(\mathbf{e};s)$
    \STATE Get verification score using Eq. (\ref{eq:verify})
\ENDFOR
\end{algorithmic}
\textbf{Output:} $s \in \mathcal{S} $ with highest verification score
\end{algorithm}




==> intro_old.tex <==
\section{Introduction}
Solving math word problems (MWP) is the task of answering a mathematical question according to textual content. It is an important and fundamental task in natural language understanding (NLU) due to its requirement on numerically reasoning. Early approaches mainly craft rules and templates for pattern matching. Later on, researchers use statistical methods to solve MWP and achieve a great performance gain. However, these methods rely heavily on feature engineering and template designing. Thus, they are only suitable for small-scale datasets.

Recently, sequence-to-sequence (Seq2Seq) models have achieved great success in many natural language processing (NLP) tasks including machine translation, summarization, and question answering. In the meantime, large-scale MWP datasets are also constructed. This leads to a new trend in MWP solvers which approach the task as the translation from problem texts to mathematical expressions. DNS is the first to apply vanilla RNN-based models to MWP. Wang et al. 2018 further compare three Seq2Seq models on MWP solving and propose an ensemble model. Some work also leverage tree structures or graph information to improve performance. Shen and Jin propose a seq2seq model with multi-encoders and multi-decoders and achieve the SOTA performance.

Although treating MWP as translation achieves promising results, there is an important difference between mathematical expressions and natural language: one mistake in an expression will change the whole semantic thus lead to a wrong answer, while natural language is more robust to minor mistakes. The objective of Seq2Seq training is to maximize the generation likelihood on ground-truth, which gives a minor penalty if the model output differs slightly from the ground-truth. This is acceptable for translation but not for MWP. Thus, this training objective is not sufficient to obtain the best MWP solvers.

Humans solve MWP more carefully than translate. After writing down an expression, they usually check the correctness of this expression and make some revisions if they find any mistakes. Inspired by this, we propose a multi-task framework where the MWP solver can learn from its own mistakes with three different tasks, namely generating, rewriting and ranking. 
% The objective of generating is the same as the vanilla Seq2Seq training where the model learns to generate an expression given the math word problem.  

Recent years also witness the great advancement of pre-trained language models such as BERT, GPT, and XLNet on various NLP tasks. There is much evidence showing that pre-trained language models learn not only contextualized text representations, but also grammar, commonsense and world knowledge. However, little effort has been made to explore their ability in solving math word problems. In this work, we use BART, a pre-trained sequence-to-sequence model, to MWP and show its superiority over other baseline models. To our knowledge, we are the first to apply pre-trained models to MWP.

In summary, the contributions of our work are as follows:

\begin{itemize}
    \vspace{-0.05in}
    \item We propose a multi-task framework to train Seq2Seq models for math word problems solving.
    \vspace{-0.1in}
    \item We are the first to apply a pre-trained language model to math word problems.
    \vspace{-0.1in}
    \item Experiments show that our proposed model achieves a significant improvement over previous state-of-the-art models.
\end{itemize}
